Search for a Low-Mass Neutral Higgs Boson with Suppressed Couplings to Fermions Using Events with Multiphoton Final States

A search for a Higgs boson with suppressed couplings to fermions, $h_f$, assumed to be the neutral, lower-mass partner of the Higgs boson discovered at the Large Hadron Collider, is reported. Such a Higgs boson could exist in extensions of the standard model with two Higgs doublets, and could be produced via $p\bar{p} \to H^\pm h_f \to W^* h_f h_f \to 4\gamma + X$, where $H^\pm$ is a charged Higgs boson. This analysis uses all events with at least three photons in the final state from proton-antiproton collisions at a center-of-mass energy of 1.96~TeV collected by the Collider Detector at Fermilab, corresponding to an integrated luminosity of 9.2~${\rm fb}^{-1}$. No evidence of a signal is observed in the data. Values of Higgs-boson masses between 10 and 100 GeV/$c^2$ are excluded at 95\% Bayesian credibility.

==> setup/symbols.tex <==
\input $TEX/symbols_physics.tex
\input $TEX/symbols_util.tex


==> setup/symbols_cdf.tex <==
%------------------------------------------------------------------------------

%-- ELECTRON_CENTRAL_18
\def \TrgEL {{\tt ELECTRON$\_$CENTRAL$\_$18}}

%-- MUON_CMUP18 trigger paths
\def \TrgUPa {{\tt MUON$\_$CMUP18}}
\def \TrgUPb {{\tt MUON$\_$CMUP18$\_$L2$\_$PT15}}
\def \TrgUPc {{\tt MUON$\_$CMUP18$\_$L2$\_$LOOSE$\_$LUMI$\_$240}}
\def \TrgUPd {{\tt MUON$\_$CMUP18$\_$L2$\_$LOOSE$\_$LUMI$\_$260}}
\def \TrgUPe {{\tt MUON$\_$CMUP18$\_$L2$\_$LOOSE$\_$DPS}}

%-- MUON_CMX18 trigger paths
\def \TrgMXa {{\tt MUON$\_$CMX18}}
\def \TrgMXb {{\tt MUON$\_$CMX18$\_$L2$\_$PT15}}
\def \TrgMXc {{\tt MUON$\_$CMX18$\_$L2$\_$PT15$\_$LUMI$\_$200}}
\def \TrgMXd {{\tt MUON$\_$CMX18$\_$L2$\_$LOOSE$\_$LUMI$\_$200}}
\def \TrgMXe {{\tt MUON$\_$CMX18$\_$L2$\_$LOOSE$\_$DPS}}
\def \TrgMXf {{\tt MUON$\_$CMX18$\_$L2$\_$PS10}}
\def \TrgMXg {{\tt MUON$\_$CMX18$\_$L2$\_$PS100}}
\def \TrgMXh {{\tt MUON$\_$CMX18$\_$LUMI$\_$250}}
\def \TrgMXi {{\tt MUON$\_$CMX18$\_$DPS}}
\def \TrgMXj {{\tt MUON$\_$CMX18$\_\&\_$JET10}}
\def \TrgMXk {{\tt MUON$\_$CMX18$\_\&\_$JET10$\_$LUMI$\_$270}}
\def \TrgMXl {{\tt MUON$\_$CMX18$\_\&\_$JET10$\_$DPS}}

%-- W_NOTRAK
\def \TrgWNT {{\tt W$\_$NOTRAK}}

%-- ELECTRON_CENTRAL_18_NO_L2
\def \TrgELNoLTwo {{\tt ELECTRON$\_$CENTRAL$\_$18$\_$NO$\_$L2}}


%-- Track quality cuts
\def \Saxst  {COT hit}
\def \SzOzpv {\wrap{z_{0}-z_{\rm pv}}}
\def \SdO    {\wrap{d_{0}}}
\def \Ssi    {Silicon hit}
\def \STrks  {Track quality cuts}
 
%-- Isolation cut
\def \Siso   {\wrap{{\rm ISO}^{\rm cal}_{0.4}}}
 
%-- Electron Idendification cuts
\def \Shadem {HAD/EM}
\def \Slshr  {\wrap{L_{\rm shr}}}
\def \Seop   {\wrap{E/p}}
\def \Schis  {\wrap{\chi^{2}_{\rm srtip}}}
\def \Sdzces {\wrap{\Delta z_{\rm CES}}}
\def \Sqdx   {\wrap{Q\times\Delta x_{\rm CES}}}
\def \Sconv  {Conversion removal}
\def \Scpr   {CPR cut}

%-- Muon Selection cuts
\def \Shad   {HAD} 
\def \Sem    {EM}  
\def \Srdphi {\wrap{r\times\Delta \phi}}

%-- Lepton Identification cuts
\def \SIDc {Identification cuts (w/o CPR)}
\def \SIDs {Identification cuts}

%-- Lepton Selection cuts
\def \SSLc {Overall (w/o CPR) }
\def \SSLs {Overall}

%-- z1-z2 cuts
\def \SdzO  {\wrap{z_{01}-z_{02}}}

%-- Dilepton type
\def \CECE {CEM-CEM}
\def \EHEL {CEM-CEM}
\def \EHEH {CEM-CEM}
\def \UPUP {CMUP-CMUP}
\def \UPMX {CMUP-CMX}
\def \UPAR {CMUP-CMX(AR)}
\def \UPKS {CMUP-CMX(KS)}
\def \UPMS {CMUP-CMX(MS)}
\def \MXUP {CMX-CMUP}
\def \MXMX {CMX-CMX}
\def \MXAR {CMX-CMX(AR)}
\def \MXKS {CMX-CMX(KS)}
\def \MXMS {CMX-CMX(MS)}

%-- Smaples
\def \Ze {Drell-Yan (\wrap{Z/\gamma^{\ast}\rightarrow e^{+}e^{-}})}
\def \Zm {Drell-Yan (\wrap{Z/\gamma^{\ast}\rightarrow \mu^{+}\mu^{-}})}
\def \Zt {Drell-Yan (\wrap{Z/\gamma^{\ast}\rightarrow \tau^{+}\tau^{-}})}
\def \Ha {higgs : \wrap{M_{{\rm higgs}} = 110 ({\rm GeV}/c^{2})}}
\def \Hb {higgs : \wrap{M_{{\rm higgs}} = 120 ({\rm GeV}/c^{2})}}
\def \Hc {higgs : \wrap{M_{{\rm higgs}} = 130 ({\rm GeV}/c^{2})}}
\def \Hd {higgs : \wrap{M_{{\rm higgs}} = 140 ({\rm GeV}/c^{2})}}
\def \He {higgs : \wrap{M_{{\rm higgs}} = 150 ({\rm GeV}/c^{2})}}
\def \Hf {higgs : \wrap{M_{{\rm higgs}} = 160 ({\rm GeV}/c^{2})}}
\def \Hg {higgs : \wrap{M_{{\rm higgs}} = 170 ({\rm GeV}/c^{2})}}
\def \Hh {higgs : \wrap{M_{{\rm higgs}} = 180 ({\rm GeV}/c^{2})}}
\def \Hi {higgs : \wrap{M_{{\rm higgs}} = 190 ({\rm GeV}/c^{2})}}
\def \Hj {higgs : \wrap{M_{{\rm higgs}} = 200 ({\rm GeV}/c^{2})}}
\def \OA {Overall}

%-- dphi(1,2)
\def \dphDL { \wrap{\Delta\phi_{\ell_{1}\ell_{2}}} }


% Z/gamma ->ll
\def \Zll {\wrap{Z/\gamma^{*}\rightarrow\ell^{+}\ell^{-}}}
\def \Zee {\wrap{Z/\gamma^{*}\rightarrow e^{+}e^{-}}}
\def \Zmm {\wrap{Z/\gamma^{*}\rightarrow\mu^{+}\mu^{-}}}

%-- bigcircle
\def \bc {\wrap{\bigcirc}}


==> setup/utils.tex <==
%==============================================================================
% Revisions:
% 01/05/05 - \blankline is changed from \vspace{\baselineskip} to 
%	     $\mbox{}$\\
%==============================================================================
\def \blankline {$\mbox{}$\\}
\def \lsim  {\mbox{ \raisebox{-.6ex}{$\stackrel{<}{\sim}$} }}
\def \upm {$\pm$}
\def \mc {\multicolumn}
\def \degr {$^{\circ}$}
\def \mdegr {^{\circ}}
\def \degrC {$^{\circ}$C}
\def \onespace     {$\:$}
\def \monespace    {\:}
\def \ds		{\displaystyle}
\def \bmath {\begin{displaymath}}
\def \emath {\end  {displaymath}}
\def \beq   {\begin{equation}}
\def \eeq   {\end  {equation}}
\def \bitem {\begin{itemize}}
\def \eitem {\end  {itemize}}
\def \benum {\begin{enumerate}}
\def \eenum {\end  {enumerate}}
\def \bcenter {\begin{center}}
\def \ecenter {\end  {center}}
\def \CommentOut#1 {\if0 #1 \fi}

\newlength{\pushupfigure}
\setlength{\pushupfigure}{-55.5pt}
\def \epsfin_v1#1#2{
	\vspace{\pushupfigure}
	\center
	\leavevmode
	\epsfxsize=#1
	\epsffile[20 143 575.75 698.75]{#2}
}
%---- 2/15/98 Noticed Latex does not recognize _ in the command. Therefore
% upgrading this command by epsfin_v2 does not work. It seems working in doing
% epsfA, epsfB, ... So let's indicate its version by a capital letter A, B, ...
%
% 11/29/05: After start using ROOT figures, we have to optimize some margins.
% Put vspace{3cm}.
%
% A = Same as \epsfin_v1
\def \epsfA#1#2{
	\vspace{\pushupfigure}
	\center
	\leavevmode
	\epsfxsize=#1
	\epsffile[20 143 575.75 698.75]{#2}
\vspace*{3cm}
}

% B = Bounding box is the same as the plot box, not the box surrounding a plot
% Also \pushupfigure is removed.
% 03/07/01 - Added 5 mm vspace below the plot
\def \epsfB#1#2{
%	\vspace{\pushupfigure}
	\center
	\leavevmode
	\epsfxsize=#1
	\epsffile[75.5 198.5 520.25 643.25]{#2}
\vspace*{5mm}
}


%---- Reserved for the future upgrade
\def \epsfC#1#2{
%	\vspace{\pushupfigure}
	\center
	\leavevmode
	\epsfxsize=#1
	\epsffile{#2}
%	\epsffile[75.5 198.75 464.75 588]{#2}
}

\def \mspace {\mbox{ }\mbox{ }\mbox{ }\mbox{ }\mbox{ }\mbox{ }}

\newlength{\figsize}
\setlength{\figsize}{\textwidth}

%------------------------------------------------------------------------------
\def \OnePlot#1{
\def \plotwidth {\linewidth}
\bcenter
\includegraphics[width=\plotwidth]{#1}
\ecenter
}
%------------------------------------------------------------------------------
\def \TwoPlots#1#2{
\def \plotwidth {0.65\linewidth}
\begin{minipage}[h]{\linewidth}
\bcenter
\includegraphics[width=\plotwidth]{#1}
\\[1cm]
\includegraphics[width=\plotwidth]{#2}
\ecenter
\end{minipage}
}
%------------------------------------------------------------------------------
\def \ThreePlots#1#2#3{
\begin{minipage}[h]{\linewidth}
\hspace{-5mm}
\includegraphics[width=\plotwidth]{#1}
\hspace{-5mm}
\includegraphics[width=\plotwidth]{#2}
\end{minipage}
\\[1cm]
\hspace{1cm}
\includegraphics[width=\plotwidth]{#3}
}
%------------------------------------------------------------------------------
\def \ThreePlotsB#1#2#3{
\hspace{1cm}
\includegraphics[width=\plotwidth]{#1}
\\[1cm]
\begin{minipage}[h]{\linewidth}
\hspace{-5mm}
\includegraphics[width=\plotwidth]{#2}
\hspace{-5mm}
\includegraphics[width=\plotwidth]{#3}
\end{minipage}
}
%------------------------------------------------------------------------------
\def \FourPlots#1#2#3#4{
\begin{minipage}[h]{\linewidth}
\hspace{-7mm}
\includegraphics[width=\plotwidth]{#1}
\hspace{-7mm}
\includegraphics[width=\plotwidth]{#2}
\end{minipage}
\\[1cm]
\begin{minipage}[h]{\linewidth}
\hspace{-7mm}
\includegraphics[width=\plotwidth]{#3}
\hspace{-7mm}
\includegraphics[width=\plotwidth]{#4}
\end{minipage}
}
%------------------------------------------------------------------------------

